House-GAN: Relational Generative Adversarial Networks for Graph-constrained House Layout Generation

This paper proposes a novel graph-constrained generative adversarial network, whose generator and discriminator are built upon relational architecture. The main idea is to encode the constraint into the graph structure of its relational networks. We have demonstrated the proposed architecture for a new house layout generation problem, whose task is to take an architectural constraint as a graph (i.e., the number and types of rooms with their spatial adjacency) and produce a set of axis-aligned bounding boxes of rooms. We measure the quality of generated house layouts with the three metrics: the realism, the diversity, and the compatibility with the input graph constraint. Our qualitative and quantitative evaluations over 117,000 real floorplan images demonstrate that the proposed approach outperforms existing methods and baselines. We will publicly share all our code and data.

==> sections/8_baselines.tex <==
\section{Additional experimental details} In the compatibility score computation  (graph edit distance), we decreased the number of test samples from 5,000 to 1,000 for graphs of size 10-12 and 13+, due to its high computational cost. For all experiments, we compute the graph edit distance score using the function \textit{optimize\_edit\_distance} from NetworkX version 2.4~\cite{hagberg2008exploring}. We set the upper bound (max distance) to 40 and added a timeout of 1 hour to this function call. In the ablation study for compatibility, the first baseline without any constraint (i.e. CNN-only without room count, type and connectivity) was evaluated disregarding the room type in the graph edit distance computation, since no room type information is estimated nor given in this baseline.

\section{Baselines architectural specification}

Tables~\ref{table:full_architecture_cnn} and~\ref{table:full_architecture_gcn} present the full architecture specification for the CNN-only and GCN baselines.

%%%%%%%%%% CNN-only architectural specification %%%%%%%%%%%%%
        % z = z.view(-1, 128)
        % if self.with_graph == True:
        %     y = given_y.view(-1, 10*self.max_nodes)
        %     given_w = given_w[:, 1]
        %     w = given_w.view(-1, self.max_edges)
        %     z = torch.cat([z, y, w], 1)
        % x = self.l1(z)
        % x = x.view(-1, 16, self.init_size, self.init_size)
        % x = self.upsample_1(x)
        % x = self.upsample_2(x)
        % x = self.decoder(x.view(-1, x.shape[1], *x.shape[2:]))
        % x = x.view(-1, *x.shape[2:])
\renewcommand{\arraystretch}{1.1}
    \begin{table*}[t]
    \caption{CNN-only architectural specification.
    %Shows architecture details for the proposed house layout generator and discriminator in Space-GAN. 
    ``s" and ``p" denote stride and padding.
    %in convolution layers. 
    Considering 40 to be the maximum number of rooms in our experiments.
    ``x", ``z", ``t" and ``c" denote the room mask, noise vector, all room types vector concatenated (i.e. $1\times400$) and all connections (i.e. 780=$40\choose 2$) represented as a 1D vector ($1\times780$). Convolution kernels and layer dimensions are specified as ($N_{in}\times N_{out} \times W \times H$) and ($W \times H \times C$).}
    %as convolution kernels and layer output dimensions, respectively.}
    \label{table:full_architecture_cnn}
    \centering
        \begin{tabular}{cccc}
        \toprule
        Architecture & Layer & Specification & Output Size\\
        \midrule
        \midrule
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%
        %%%%%%% Generator %%%%%%%%%%
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%
        & $concat(z, t, c)$ & N/A &  $1\times1308$\\
        \cmidrule{2-4}
        & $linear\_reshape_1$ & $1308\times1024$ &  $8\times8\times16$\\
        \cmidrule{2-4}
        %
        \multirow{2}{*}{\parbox{2cm}{\centering House layout\\ generator}} & $upsample_1$ & $16\times16\times4\times4, (s=2, p=1)$ &  $16\times16\times16$\\
        \cmidrule{2-4}
        %
        & $upsample_2$ & $16\times16\times4\times4, (s=2, p=1)$ &  $32\times32\times16$\\
        \cmidrule{2-4}
        & $conv\_leaky\_relu_1$ & $16\times256\times3\times3, (s=1, p=1)$ &  $32\times32\times256$\\
        \cmidrule{2-4}
        %
        & $conv\_leaky\_relu_2$ & $256\times128\times3\times3, (s=1, p=1)$ &  $32\times32\times128$\\
         \cmidrule{2-4}
        %
        & $conv\_tanh_1$ & $128\times40 \times3\times3, (s=1, p=1)$ &  $32\times32\times40$\\
        \midrule
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        %%%%%%% Discriminator %%%%%%%%%%
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        & $concat(t, c)$ & N/A &  $1\times1180$\\
        \cmidrule{2-4}
        & $linear\_reshape_1$ & $1180\times8192$ &  $32\times32\times8$\\
        \cmidrule{2-4}
        %
        & $concat\_with(x)$ & N/A &  $32\times32\times9$\\
        \cmidrule{2-4}
        %
        & $conv\_leaky\_relu_1$ & $9\times16\times3\times3, (s=1, p=1)$ &  $32\times32\times16$\\
        \cmidrule{2-4}
        %
        & $conv\_leaky\_relu_2$ & $16\times16\times3\times3, (s=1, p=1)$ &  $32\times32\times16$\\
        \cmidrule{2-4}
        %
        \multirow{2}{*}{\parbox{2cm}{\centering House layout\\ discriminator}} & $conv\_leaky\_relu_3$ & $16\times16\times3\times3, (s=1, p=1)$ &  $32\times32\times16$\\
        \cmidrule{2-4}
        %
        & $downsample_1$ &  $16\times16\times3\times3, (s=2, p=1)$ &  $16\times16\times16$\\
        \cmidrule{2-4}
        %
        & $downsample_2$ &  $16\times16\times3\times3, (s=2, p=1)$ &  $8\times8\times16$\\
        \cmidrule{2-4}
        %
        & $conv\_leaky\_relu_1$ & $16\times256\times3\times3, (s=2, p=1)$ &  $4\times4\times256$\\
        \cmidrule{2-4}
        %
        & $conv\_leaky\_relu_2$ & $256\times128\times3\times3, (s=2, p=1)$ &  $2\times2\times128$\\
        \cmidrule{2-4}
        %
        & $conv\_leaky\_relu_3$ & $128\times128\times3\times3, (s=2, p=1)$ &  $1\times1\times128$\\
        \cmidrule{2-4}
        %
        & $reshape\_linear_1$ & $128\times1$ &  $1$\\
        \bottomrule
        \end{tabular}
    \end{table*}

%%%%%%%%%% GCN architectural specification %%%%%%%%%%%%
\renewcommand{\arraystretch}{1.1}
    \begin{table*}[t]
    \caption{GCN architectural specification.
    %Shows architecture details for the proposed house layout generator and discriminator in Space-GAN. 
    ``s" and ``p" denote stride and padding.
    %in convolution layers. 
    ``x", ``z" and ``t" denote room mask, noise vector, and room type vector. ``gcn" layers are implemented using the official code borrowed from Ashual~\etal~\cite{ashual2019specifying} and Johnson~\etal~\cite{johnson2018image}. In ``gcn", $d_{in}$ denotes input dimension, $d_{h}$ hidden dimension and $n_{l}$ number of layers. All ``gcn" layers uses average pooling. Convolution kernels and layer dimensions are specified as ($N_{in}\times N_{out} \times W \times H$) and ($W \times H \times C$).}
    %as convolution kernels and layer output dimensions, respectively.}
    \label{table:full_architecture_gcn}
    \centering
        \begin{tabular}{cccc}
        \toprule
        Architecture & Layer & Specification & Output Size\\
        \midrule
        \midrule
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%
        %%%%%%% Generator %%%%%%%%%%
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%
        & $concat(z, t)$ & N/A &  $1\times138$\\
        \cmidrule{2-4}
        & $linear_1$ & $138\times128$ &  $1\times128$\\
        \cmidrule{2-4}
        %
        & $gcn$ & $(d_{in}=128,d_{h}=512,n_{l}=2)$ &  $1\times128$\\
        \cmidrule{2-4}
        %
        \multirow{2}{*}{\parbox{2cm}{\centering House layout\\ generator}} & $linear_2\_reshape$ & $128\times1024$ &  $8\times8\times16$\\
        \cmidrule{2-4}
        %
        & $upsample_1$ & $16\times16\times4\times4, (s=2, p=1)$ &  $16\times16\times16$\\
        \cmidrule{2-4}
        %
        & $upsample_2$ & $16\times16\times4\times4, (s=2, p=1)$ &  $32\times32\times16$\\
        \cmidrule{2-4}
        & $conv\_leaky\_relu_1$ & $16\times256\times3\times3, (s=1, p=1)$ &  $32\times32\times256$\\
        \cmidrule{2-4}
        %
        & $conv\_leaky\_relu_2$ & $256\times128\times3\times3, (s=1, p=1)$ &  $32\times32\times128$\\
         \cmidrule{2-4}
        %
        & $conv\_tanh_1$ & $128\times1\times3\times3, (s=1, p=1)$ &  $32\times32\times1$\\
        \midrule
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        %%%%%%% Discriminator %%%%%%%%%%
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        & $linear\_reshape_1(t)$ & $10\times8192$ &  $32\times32\times8$\\
        \cmidrule{2-4}
        %
        & $concat(t, x)$ & N/A &  $32\times32\times9$\\
        \cmidrule{2-4}
        %
        & $conv\_leaky\_relu_1$ & $9\times16\times3\times3, (s=1, p=1)$ &  $32\times32\times16$\\
        \cmidrule{2-4}
        %
        & $conv\_leaky\_relu_2$ & $16\times16\times3\times3, (s=1, p=1)$ &  $32\times32\times16$\\
        \cmidrule{2-4}
        %
        & $conv\_leaky\_relu_3$ & $16\times16\times3\times3, (s=1, p=1)$ &  $32\times32\times16$\\
        \cmidrule{2-4}
        %
        \multirow{2}{*}{\parbox{2cm}{\centering House layout\\ discriminator}} & $downsample_1$ &  $16\times16\times3\times3, (s=2, p=1)$ &  $16\times16\times16$\\
        \cmidrule{2-4}
        %
        & $downsample_2$ &  $16\times16\times3\times3, (s=2, p=1)$ &  $8\times8\times16$\\
        \cmidrule{2-4}
        %
        & $conv\_leaky\_relu_1$ & $16\times256\times3\times3, (s=2, p=1)$ &  $4\times4\times256$\\
        \cmidrule{2-4}
        %
        & $conv\_leaky\_relu_2$ & $256\times128\times3\times3, (s=2, p=1)$ &  $2\times2\times128$\\
        \cmidrule{2-4}
        %
        & $conv\_leaky\_relu_3$ & $128\times128\times3\times3, (s=2, p=1)$ &  $1\times1\times128$\\
        \cmidrule{2-4}
        %
        & $gcn$ & $(d_{in}=128,d_{h}=512,n_{l}=2)$ &  $1\times128$\\
        \cmidrule{2-4}
        %
        & $pool\_reshape\_linear_1$ & $128\times1$ &  $1$\\
        \bottomrule
        \end{tabular}
    \end{table*}


==> sections/9_additional_results.tex <==
\section{Additional results}
Figures \ref{fig:results_1}-\ref{fig:results_10} present additional generation results by the proposed system (House-GAN). Each row shows an input bubble diagram and pairs of a generated room mask and the corresponding house layout.
%generated room masks and their corresponding house layout by the proposed approach (House-GAN).
We divide the samples into 5 groups depending on the numbers of rooms. We present two pages of results for each group, in a increasing order of the room counts.
%instance of House-GAN trained and tested on graphs of different sizes.

% xxxxxxxx MENTION that now different figures show graphs with different sizes... xxxxx
%instance trained and tested on graphs of size 1-12 and 13+, respectively. 


\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{images/page_1_A.png}
\caption{Additional qualitative results for room masks and final house layouts. Each row shows four generated sample pairs (i.e. mask and layout) for the same graph presented in the first column. Model was trained on graphs of size 4+ and tested on graphs of size 1-3.}
\label{fig:results_1}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{images/page_2_A.png}
\caption{Continued.}
\label{fig:results_2}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{images/page_1_B.png}
\caption{Results for model trained on graphs of size 1-3 and 7+ and tested on graphs of size 4-6.}
\label{fig:results_3}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{images/page_2_B.png}
\caption{Continued.}
\label{fig:results_4}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{images/page_1_C.png}
\caption{{Results for model trained on graphs of size 1-6 and 10+ and tested on graphs of size 7-9.}}
\label{fig:results_5}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{images/page_2_C.png}
\caption{Continued.}
\label{fig:results_6}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{images/page_1_D.png}
\caption{Results for model trained on graphs of size 1-9 and 13+ and tested on graphs of size 10-12.}
\label{fig:results_7}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{images/page_2_D.png}
\caption{Continued.}
\label{fig:results_8}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{results/page_6.png}
\caption{Results for model trained on graphs of size 1-12 and tested on graphs of size 13+.}
\label{fig:results_9}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{results/page_1.png}
\caption{Continued.}
\label{fig:results_10}
\end{figure*}


